A Simple and Realistic Pedestrian Model for Crowd Simulation and Application

The simulation of pedestrian crowd that reflects reality is a major challenge for researches. Several crowd simulation models have been proposed such as cellular automata model, agent-based model, fluid dynamic model, etc. It is important to note that agent-based model is able, over others approaches, to provide a natural description of the system and then to capture complex human behaviors. In this paper, we propose a multi-agent simulation model in which pedestrian positions are updated at discrete time intervals. It takes into account the major normal conditions of a simple pedestrian situated in a crowd such as preferences, realistic perception of environment, etc. Our objective is to simulate the pedestrian crowd realistically towards a simulation of believable pedestrian behaviors. Typical pedestrian phenomena, including the unidirectional and bidirectional movement in a corridor as well as the flow through bottleneck, are simulated. The conducted simulations show that our model is able to produce realistic pedestrian behaviors. The obtained fundamental diagram and flow rate at bottleneck agree very well with classic conclusions and empirical study results. It is hoped that the idea of this study may be helpful in promoting the modeling and simulation of pedestrian crowd in a simple way.

==> 2B_AgentBasedModel.tex <==
%%%%%%%%%% Agent-Based Models %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Conf1:2D
\subsection{Agent-Based Model}\label{sec:II_B}
%
% Conf1:2D
An agent-based model
%
%\cite{ref:agent1, ref:agent2, ref:SCI1-31, ref:SCI1-32, ref:SCI1-33,
%ref:SCI1-34, ref:Conf1-5, ref:Conf1-24, ref:Conf1-25, ref:Conf1-26,
%ref:Conf1-27}
%
\cite{ref:Conf1-3, ref:agent2} is a
%
collection of autonomous and intelligent agents. Each agent has a
set of characteristics such as mobility, walking speed, and moving
direction. These characteristics can change depending on the agent
situation and the environment. The pedestrian agent can take its
decisions and actions through simple internal rules. Thus, the
agent-based models are able, over others approaches, to be flexible,
to provide a natural description of the system, and to capture
complex human behaviors \cite{ref:Conf1-3}. In other words, they may
reflect more the reality.

% Conf1:2D
Usually, these models are based on mathematical equations that have
to reproduce pedestrian crowd laws. However, human behaviors are so
complex that it is sometimes difficult to capture them as
mathematical equations \cite{ref:Conf1-28}. For this reason, and in
order to obtain a more realistic simulation of pedestrian behaviors,
several models based on agents and various human nature factors have
been proposed \cite{ref:SCI1-31, ref:SCI1-32, ref:SCI1-34}.
% \cite{ref:Conf1-5, ref:Conf1-24, ref:Conf1-26}.
%
% Conf1:2D
% However, a great number of these models do not cover all the factors
% necessary for a pedestrian crowd. Therefore the produced pedestrian
% crowd situations lack realism.
